Modeling the Background for Incremental Learning in Semantic Segmentation

Despite their effectiveness in a wide range of tasks, deep architectures suffer from some important limitations. In particular, they are vulnerable to catastrophic forgetting, i.e. they perform poorly when they are required to update their model as new classes are available but the original training set is not retained. This paper addresses this problem in the context of semantic segmentation. Current strategies fail on this task because they do not consider a peculiar aspect of semantic segmentation: since each training step provides annotation only for a subset of all possible classes, pixels of the background class (i.e. pixels that do not belong to any other classes) exhibit a semantic distribution shift. In this work we revisit classical incremental learning methods, proposing a new distillation-based framework which explicitly accounts for this shift. Furthermore, we introduce a novel strategy to initialize classifier's parameters, thus preventing biased predictions toward the background class. We demonstrate the effectiveness of our approach with an extensive evaluation on the Pascal-VOC 2012 and ADE20K datasets, significantly outperforming state of the art incremental learning methods.

==> ade-pc-results.tex <==
\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{3pt} % Default value: 6pt
\caption{Mean IoU on the first order of ADE20K dataset for different incremental class learning scenarios.}
\label{tab:ade}
\begin{tabular}{l||cc|c||cccccc|c||ccc|c}
\multicolumn{1}{c}{} & \multicolumn{3}{c}{{\textbf{100-50}}} & \multicolumn{7}{c}{{\textbf{100-10}}} & \multicolumn{4}{c}{{\textbf{50-50}}} \\
\textbf{Method}       & \textit{1-100} & \textit{101-150} & \textit{all}  & \textit{1-100} & \textit{100-110} & \textit{110-120} & \textit{120-130} & \textit{130-140} & \textit{140-150} & \textit{all}  & \textit{1-50} & \textit{51-100} & \textit{101-150} & \textit{all}  \\ \hline
FT      & 0.0   & 18.7    & 6.2  & 0.0   & 0.0    & 0.0    & 0.0    & 0.0    & \textbf{11.5}   & 0.8  & 0.0  & 0.0    & 17.5    & 5.8  \\
LwF     & 23.6  & 18.2    & 21.8 & 0.2   & 0.0    & 0.8    & 1.5    & 1.5    & 10.7   & 1.1  & 6.3  & 15.3   & 16.0    & 12.6 \\
LwF-MC  & \textbf{42.0}  & 4.8     & 29.6 & 25.8  & \textbf{1.5}    & \textbf{10.6}   & 1.7    & 3.0    & 0.0    & 18.3 & 27.8 & 7.0    & 10.4    & 15.1 \\
ILT     & 25.3  & 11.2    & 20.6 & 0.4   & 0.0    & 1.9    & 0.6    & 1.6    & 3.3    & 0.7  & 8.6  & 10.3   & 8.3     & 8.9  \\
MiB     & 41.5  & \textbf{22.1}    & \textbf{35.0} & \textbf{37.8}  & 1.3    & 8.8    & \textbf{9.9}    & \textbf{5.1}    & 10.5   & \textbf{27.6} & \textbf{45.3} & \textbf{21.0}   & \textbf{18.5}    & \textbf{27.9} \\ \hline
Joint   & 44.3  & 28.2    & 38.9 & 44.3  & 26.1   & 42.8   & 26.7   & 28.1   & 17.3   & 38.9 & 51.1 & 38.3   & 28.2    & 38.9
\end{tabular}
\end{table*}

\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{3pt} % Default value: 6pt
\caption{Mean IoU on the second order of ADE20K dataset for different incremental class learning scenarios.}
\label{tab:ade}
\begin{tabular}{l||cc|c||cccccc|c||ccc|c}
\multicolumn{1}{c}{} & \multicolumn{3}{c}{{\textbf{100-50}}} & \multicolumn{7}{c}{{\textbf{100-10}}} & \multicolumn{4}{c}{{\textbf{50-50}}} \\
\textbf{Method}       & \textit{1-100} & \textit{101-150} & \textit{all}  & \textit{1-100} & \textit{100-110} & \textit{110-120} & \textit{120-130} & \textit{130-140} & \textit{140-150} & \textit{all}  & \textit{1-50} & \textit{51-100} & \textit{101-150} & \textit{all}  \\ \hline
FT     & 0.0   & 31.2    & 10.4 & 0.0   & 0.0    & 0.0    & 0.0    & 0.0    & 21.6   & 1.4  & 0.0  & 0.0    & 26.6    & 8.9  \\
LwF    & 18.5  & 33.0    & 23.4 & 0.0   & 0.0    & 0.0    & 3.7    & 7.7    & 23.1   & 2.3  & 5.1  & 10.6   & \textbf{29.5}    & 15.2 \\
LwF-MC & 26.4  & 16.2    & 23.0 & 11.7  & 3.5    & 6.7    & 6.5    & 9.9    & 10.1   & 10.2 & \textbf{27.8} & 7.0    & 10.4    & 15.1 \\
ILT    & 20.6  & 26.6    & 22.6 & 0.2   & 0.0    & 0.0    & 3.6    & 7.7    & 18.1   & 2.1  & 8.3  & 9.1    & 20.3    & 12.7 \\
MiB    & \textbf{34.2}  & \textbf{33.8}    & \textbf{34.1} & \textbf{25.8}  & \textbf{19.6}   & \textbf{20.9}   & \textbf{15.8}   & \textbf{22.0}   & \textbf{26.9}   & \textbf{24.2} & 25.7 & \textbf{23.4}   & 28.6    & \textbf{26.2} \\ \hline
Joint  & 44.3  & 28.2    & 38.9 & 44.3  & 26.1   & 42.8   & 26.7   & 28.1   & 17.3   & 38.9 & 51.1 & 38.3   & 28.2    & 38.9 
\end{tabular}
\end{table*}

==> method_old.tex <==
\section{Method}
\label{sec:method}
In the following, we first formalize the problem of incremental learning for semantic segmentation (Sec. \ref{sec:problem}) and describe how this task can be addressed with a knowledge distillation-based approach (Sec. \ref{sec:standard-kd}). Then, in Sec. \ref{sec:our-method} we introduce the proposed approach for incremental learning by explicitly modelling background information.

\subsection{Problem Definition and Notation}
\label{sec:problem}
In this work we address the problem of incremental class learning for semantic segmentation. In particular, our goal is to progressively augment the output space of a pretrained segmentation model with novel classes for which no labeled data was available in the initial training phase. Furthermore, we assume that, while learning the novel categories, the initial training set is unavailable. This introduces an inherent bias of the learned model towards the novel classes, %which in turns causes 
eventually leading to the issue of catastrophic forgetting.
%The goal of semantic image segmentation is to assign a semantic label to each pixel of an image. 

%\textbf{Incremental Learning for Semantic Segmentation}
Before delving into the details of incremental class learning for semantic segmentation, we first introduce the task of semantic segmentation.
%Given a predetermined set of $C$ semantic
%classes encoded by $\mathcal{Y}= \{1,\dots, C\}$, 
Let us denote as $\mathcal{X}$ the input space (\ie the image space) and, without loss of generality, let us assume that each image $x\in\mathcal{X}$ is composed by a set of pixels $\set I$ with constant cardinality $N$. The goal of semantic segmentation is to assign each pixel $x_i$ of a given image $x$ a label $y_i \in \mathcal{Y}$, from some label space $\set Y$,
representing its semantic class. Out-of-class pixels can be assigned a special class, \ie the background class $\mathtt{b}\in\set Y$. The output space is a segmentation mask $(\mathcal{Y})^{N}$, with the latter denoting the product set of $N$-tuples with elements in $\mathcal{Y}$. The mapping is realized by learning a model $f_{\theta}$ with parameters $\theta$ from the image pixels space 
$\mathcal{X}$ to their corresponding segmentation mask $(\mathcal{Y})^{N}$, \ie $f_{\theta} : \mathcal{X} \mapsto (\mathcal{Y})^{N}$, given a training set $\mathcal{T} \subset \mathcal{X}\times (\mathcal{Y})^N$. %Here $(\mathcal{Y})^{N}$ denotes the n-tuple \samuel{Output space è sbagliato per segmentazione}

In the incremental learning setting, training is realized over multiple phases, called \textit{learning steps}, and each step might introduce novel categories to be learnt. In other terms, during the $t$th learning step, the previous label set $\set Y^{t-1}$ is expanded with a set of new labels $\set C^t$, yielding a new label set $\set Y^t=\set Y^{t-1}\cup\set C^{t}$.
%, each corresponding to expanding the set of possible object categories, \ie for each step $t$ the output space $\mathcal{Y}^{t}= \mathcal{Y}^{t-1} \cup \mathcal{C}^t$ where $\mathcal{C}^t$ is the set comprising to the novel categories.
%Let us call each expansion of the model with a new set of classes as \textit{learning step}, with the initial training phase denoted as \textit{step 0}. 
At learning step $t$ we are also provided with a training set $\mathcal{T}^t \subset \mathcal{X}\times (\set {C}^{t})^N$ that is used in conjunction to the previous model $f_{\theta_{t-1}}:\set X\mapsto (\set Y^{t-1})^N$ to train an updated model $f_{\theta_{t}}:\set X\mapsto(\set Y^{t})^N$.
%The starting point of a learning step $t$ is a set of parameters $\theta_{t-1}$ corresponding to the model $f_{\theta_{t-1}}: \mathcal{X} \mapsto \mathcal{Y}^{t-1}$, while the output is $\theta_t$ associated to $f_{\theta_t}$ and $\mathcal{Y}^t$. 
%, where %$\theta_{t-1}$ is the set of learned parameters, $\mathcal{X}$ is the image space and $\mathcal{Y}^{t-1}_0$ is the output space at the previous learning step. In this context, 
%$\mathcal{Y}^{t-1}$ is the set of possible pixel-wise labelling using all the known classes accumulated from learning step $0$ to $t-1$. In particular, if we denote as $\mathcal{C}^t$ the set of semantic classes relative to the learning step $t$, the set of all known classes at a learning step $t$ is $\mathcal{K}^t = \cup_{i=0}^{t}\mathcal{C}^i$.
%Notice that for two different learning steps we assume that the corresponding $\mathcal{C}^j$ %set of classes 
%share only one semantic category: the special void/background class $\mathtt{b}$, \ie $\mathcal{C}^j \cap \mathcal{C}^k = \mathtt{b}$ if $j\neq k$. 
In this paper we assume that the sets of labels $C^t$ that we obtain at the different learning steps are disjoint, except for the special void/background class $\con b$. \massi{Qui potremmo stressare che l'assunzione è ragionevole etc.}

%The output of the learning step $t$ is a set of parameters $\theta_t$ of a model $f_{\theta_t}$ mapping images to their corresponding pixel-wise labelling containing all known classes, \ie $f_{\theta_t} : \mathcal{X} \mapsto \mathcal{Y}^t_0$.

%In order to expand the semantic space of our model and learn $\theta_t$, we have a training set $\mathcal{T}^t \subset \mathcal{X}\times \mathcal{Y}^{t}_{t}$, where the output space $\mathcal{Y}_t^t$ contains pixels labeled with the only semantic classes in $\mathcal{C}^t$: no annotation is provided for the classes in $\mathcal{K}^{t-1}$, which are thus denoted as background $\mathtt{b}$. 


% Each learning step $t$ contains a set of classes $\mathcal{C}_t$ and a training set $\mathcal{T}_t \subset \mathcal{X}\times \mathcal{Y}_t$, with $\mathcal{X}$ and $\mathcal{Y}_t$ the input and output space respectively. The input space $\mathcal{X}$ is composed by the set of all possible images. Without loss of generality, we assume that each image is composed by a set of pixel $\mathcal{I}$ with constant cardinality $N=|\mathcal{I}|$. Similarly, the output space $\mathcal{Y}_t$ is composed by all the possible pixel-wise labelling of the $N$ pixels by using the classes of the $t_{th}$ step. Notice that some pixels might not belong to any of the classes in $\mathcal{C}_t$: we associate them to the void/background class ${b}$. Denoting by $\mathcal{\bar{C}}_t=\{\mathcal{C}_t,b\}$ and $y\in \mathcal{Y}_t$, we have $y^i \in \mathcal{\bar{C}}_t$ for each $i\in\mathcal{I}$. Due to the constraints of the incremental class learning scenario, given two different steps $i$ and $j$ we have that $\mathcal{C}_i \cap \mathcal{C}_j = \emptyset$ and, consequently,  $\mathcal{T}_i \cap \mathcal{T}_j = \emptyset$. 

% Each incremental step $t$ starts with a set of parameters $\theta_o=\theta_{t-1}$ and a set of known classes $\bar{\mathcal{K}}=\bar{\mathcal{K}}_{t-1} = \{\mathcal{K}_{t-1}, b\}$, with $\mathcal{K}_{t-1} = \{C_0,\dots,C_{t-1}\}$. For each incremental step, our goal is to extend $\mathcal{K}$ to $\mathcal{K}_t = \{\mathcal{K}_{t-1},C_{t}\}$ by updating $\theta_o$ into a new set of learned parameters $\theta$.
% Given a series of $T$ incremental learning steps, our goal is to learn the parameters $\theta$ of a model $f_\theta$ mapping images to their corresponding pixel-wise labelling, \ie $f_\theta : \mathcal{X} \mapsto \mathcal{Y}_T$, with $\mathcal{Y}_T$ the output space of all known classes $\mathcal{K}_T$ at time $T$, \ie $\mathcal{Y}_T=\bar{\mathcal{K}}_T^n$ with $\bar{\mathcal{K}}_T=\{\mathcal{K}_T,b\}=\{C_0,\dots,C_T,b\}$.


\subsection{Incremental Learning for Semantic Segmentation with Background Modeling}
\label{sec:standard-kd}
A naive approach to address the incremental learning problem consists in 
retraining the model $f_{\theta_t}$ on each set $\mathcal{T}^t$ sequentially. If \eg $f_{\theta_t}$ is realized through a deep architecture, this corresponds to fine-tuning the network parameters on the training set $\mathcal{T}^t$ initialized with the parameters $\theta^{t-1}$ from the previous stage. Our objective function takes the form:

\begin{equation}
   \label{eq:obj-gen}
    \mathcal{L}(\theta^t)= \frac{1}{|\mathcal{T}^t| %N M 
    }\sum_{(x,y)\in\mathcal{T}^t}
    \ell^{\theta_t}(x,y)
\end{equation}

This approach is simple, but it leads to catastrophic forgetting. Indeed, when training using $\mathcal{T}^t$ no sample from the previously-seen object classes %in $\mathcal{C}^{t-1}$, $\mathcal{C}^{t-2}$, $\dots$ 
is provided. This clearly biases the new predictor $f_{\theta_t}$ %obtained with \eqref{eq:obj-ft} 
towards the novel set of categories in $\mathcal{C}^t$ to the detriement of the classes from the previous sets. To tackle this problem, different works in incremental learning for classification \cite{li2017learning,rebuffi2017icarl,castro2018end} proposed to add to the objective loss a regularization term based on the notion of distillation \cite{hinton2015distilling}.
\textcolor{red}{qui un po' peggio di prima perchè sembra che altri lo fanno per segmentation che non è vero. ma magari basta rifrasare}


In more details, previous works proposed to address the problem of catastrophic forgetting by minimizing an objective function defined as follows:
\begin{equation}
   \label{eq:obj-ft}
    \mathcal{L}(\theta^t)= \frac{1}{|\mathcal{T}^t| %N M 
    }\sum_{(x,y)\in\mathcal{T}^t}
    \left(\ell^{\theta_t}_{ce}(x,y) + \lambda \ell^{\theta_t}_{kd}(x) \right)
\end{equation}
where  $\lambda>0$ is a parameter tuning the relative importance of two terms. The first term 
$\ell_{ce}$ is the standard cross-entropy loss over all the image pixels: 
\begin{equation}
   \label{eq:CE}
 \ell^{\theta_t}_{ce}(x,y) = -\frac{1}{|\set I|}\sum_{i \in\set I^t}\sum_{c \in\mathcal{Y}^t} y^i_c \log \sigma_{t}(f_{\theta_t}(x))^i_c
\end{equation}
\samuel{Qui assumiamo che f sputi fuori logits, ma è inconsistente con quanto scritto prima. Inoltre forse andrebbe già contestualizzato a segmentazione}
with $\sigma_t$ the softmax operation over all classes in $\mathcal{{Y}}^t$. The distillation loss $\ell_{kd}$ is defined as:
\begin{equation}
    \label{eq:std-distill}
    \ell_{kd}(x)=-\sum_{c \in \mathcal{{Y}}^{t-1}} q_{t-1}(x)_c\log q_t^\prime(x)_c
\end{equation}
where $q_{t-1}(x)=\sigma_{t-1} (f_{\theta_{t-1}}(x))$ and $q_t^\prime(x)$ are the output probabilities of the current model by applying the softmax operator only on old classes, \ie $q_t^\prime(x)=\sigma_{t-1} (f_{\theta_t}(x))$. %In \eqref{eq:obj-ft}, $\lambda$ is a trade-off parameter between the two losses. 

The rationale behind $\ell_{kd}$ is that the novel parameters should produce activations close to the ones produced by the parameters of the previous learning step. This allows to regularize the training procedure in such a way that the parameters are still anchored to the solution found for recognizing pixels of the previous classes. %Notice indeed that the softmax function is here defined across the set of classes known before starting the training step $t$, ignoring all the novel classes $\mathcal{C}_t$ added in $f_{\theta_n}$. 
The loss defined in \eqref{eq:std-distill} has been used either in its base form or variants in different works, both for incremental task \cite{li2017learning} or class learning \cite{rebuffi2017icarl,castro2018end} for classification and in complex tasks such as detection \cite{shmelkov2017incremental} and segmentation \cite{michieli2019incremental}. Despite its success, it has a fundamental drawback in our scenario: this completely ignores the fact that the background class is shared among the various learning steps and that it might contain pixels of old/novel classes. In the following section we describe how we incorporate the background in a principled way within the incremental learning steps.%in both the distillation loss defined in \eqref{eq:std-distill} and cross-entropy loss defined in \eqref{eq:CE}.

%\textcolor{red}{Notice that in distill} we have dropped the xel-wise notation for sake of simplicity and we will keep this simplification now on.

 %we assume, without loss of generality, that each image in the training set is composed by $N$ pixels a set of pixel $\mathcal{I}$ with constant cardinality $N=|\mathcal{I}|$.where $M$ is the number of pairs image-label in the training set $\mathcal{T}^t$ and $f_\theta(x)^i$ and $y^i$ denote respectively the logits and label for pixel $i \in \mathcal{I}$. In \ref{eq:obj-ft},

 % $\mathcal{K}^{t-1}$. % In the next section, we will describe a simple solution to avoid this problem based on knowledge distillation \cite{hinton2015distilling}. 

%Without loss of generality, we assume that each image is composed of a set of pixels $\mathcal{I}$, with fixed dimension $n=|\mathcal{I}|$, thus $\mathcal{X}\subset \Re^n$. Similarly, let us denote as $\mathcal{C}_k$ the set of known semantic classes. Notice that some pixels could not belong to any of the classes in $\mathcal{C}_k$: these pixels are associated to the void/background class ${b}$. By denoting $\mathcal{\bar{C}}_k=\{\mathcal{C}_k,b\}$, the output space $\mathcal{Y}_k$ is defined as the possible pixel-wise labelling, \ie $\mathcal{Y}_k=\mathcal{\bar{C}}_k^n$. Given these definitions, our goal is to learn the parameters $\theta$ of a model $f_\theta$ mapping images to their corresponding pixel-wise labelling, \ie $f_\theta : \mathcal{X} \mapsto \mathcal{Y}_k$.

% Given a training set $\mathcal{T} \subset \mathcal{X}\times \mathcal{Y}$, our goal is to  . While in the standard offline learning scenario, $\mathcal{T}$ is unique and fully available during the single training stage, here we focus on the incremental learning scenario ()However, since we are in the incremental class learning scenario, our $\mathcal{T}$ is actually divided in multiple steps This goal is usually achieved by minimizing a pixel-wise loss function such as the cross-entropy loss among the predictions of $f_\theta(x)$ and the target:
% \begin{equation}
%     \mathcal{L}(\theta, \mathcal{T}) = \frac{1}{|\mathcal{T}|\;|\mathcal{I}|}\sum_{(x,y)\in\mathcal{T}}\sum_{i\in \mathcal{I}} \ell(f_\theta(x)^i,y^i)
% \end{equation}
% where $\mathcal{I}$ is the set of pixels within an image which, without loss of generality, we assume to be same for all $x\in\mathcal{X}$, while $f_\theta(x)^i$ and $y^i$ denote respectively the prediction and label for pixel $i \in \mathcal{I}$. A standard choice for $l(\hat{y},y)$ is the cross entropy-loss:
% \begin{equation}
% l(\hat{y},y) = \sum_{c\in\mathcal{C}} y_c \log \hat{y}_c
% \end{equation}



 %Let us denote as $\theta_o$ the parameters obtained after the last incremental step and as $\theta_n$ the parameters we are currently learning. Moreover, let us define as $q_m^s(x)=\sigma_s (f_{\theta_m}(x))$ the predictions of the function $f$ obtained with the parameters $\theta_m$ and normalized according to the softmax function over $\mathcal{\bar{K}}_s$. 


\subsection{Incremental Learning for Semantic Segmentation with Background Modeling}
\label{sec:our-method}
As described in \ref{sec:problem}, differently from standard incremental class learning settings considered for image classification, in semantic segmentation we have that two different learning steps share the void/background class $\mathtt{b}$. % $\mathcal{C}_i\cap\mathcal{C}_j=\mathtt{b}$ because in all sets there could be pixels without any known label and thus assigned to the background class. 
However, %it is easy to spot that 
it is reasonable to assume that the distribution of the background class is changing across different incremental steps (\textcolor{red}{see Fig. to illustrate the intuition}). In fact, background pixels in $\mathcal{Y}^{t-1}$ could have been assigned to a class in $\mathcal{C}^t$ and vice-versa. In the following, we show how we can account for the semantic shift in the background class by modifying the supervised cross-entropy (Eq.\eqref{eq:CE}) and the distillation loss (Eq.\eqref{eq:std-distill}) and, thus, how we effectively tackle the incremental class learning problem in semantic segmentation. We also describe an effective strategy for initializing, at each learning step $t$, the parameters of the classifier for the newly introduced classes.

\myparagraph{Revisiting Cross-Entropy Loss. } The set $\mathcal{T}^t$ we use to update the learning model in each learning step $t$ only contains information about novel classes $\mathcal{C}^t$. However, the background class in $\mathcal{T}^t$ might include also pixels associated to the previously seen classes in $\mathcal{Y}^{t-1}$. In this paper we argue that, without explicitly taking into account this aspect, the catastrophic forgetting problem would be even more severe. In fact, we would drive our model to predict the background label $\mathtt{b}$ for pixels of old classes, further degrading the capability of the model to preserve semantic knowledge of past categories. To avoid this issue, in this paper we propose to modify the cross-entropy loss in Eq. \eqref{eq:CE} as follows: 
\begin{equation}
   \label{eq:our-CE}
 \ell_{uce}(x,y) = \sum_{c \ \in \ \mathcal{C}^t} y_c \log \tilde{q}_t(x)_c
 \end{equation}
 where:
\begin{equation}
    \label{eq:cases-ce}
    \begin{cases}
      \tilde{q}_t(x)_c={q}_t(x)_c\;\;& \text{if}\ c\neq\mathtt{b}\\
      \tilde{q}_t(x)_c= \sum_{k\in\mathcal{{Y}}^{t-1}}{q}_t(x)_k\;\;& \text{if}\ c=\mathtt{b}
    \end{cases}
\end{equation}

Our intuition is that by using Eq.   \eqref{eq:our-CE} we can update the model to predict the new classes and, at the same time, account for the uncertainty in the actual content of the background class. In fact, in Eq.\eqref{eq:our-CE} the background class ground truth $y_\mathtt{b}$ is not directly compared with its probabilities obtained from $f_{\theta_t}$, but with the probability of having \textit{either an old class or the background}, as predicted by $f_{\theta_t}$ (Eq.\eqref{eq:cases-ce}).% This solution allows to model the fact that a pixel labeled as background in $\mathcal{T}^t$ may actually belong to any of the classes not in $\mathcal{C}^t$ or the background itself: this produces a positive effect by both (i) avoiding a bias on $\mathtt{b}$ and (ii) mitigating the catastrophic forgetting problem.

%Notice that, without taking into account the uncertainty in $\mathtt{b}$, we would risk to have the probability of old classes harm the performances on already known classes. Indeed, if we apply \eqref{eq:CE} over a pixel labeled as background for $\mathcal{C}^t$ but actually containing a class in $\mathcal{K}_t$ we will make more severe the catastrophic forgetting problem, since features of old classes will be associated with the background classifier. 
It is worth noting that the alternative of ignoring the background pixels within the cross-entropy loss is a sub-optimal solution. In fact, this would not allow to adapt the background classifier to its semantic shift and to exploit the information that new images might contain on old classes. %Employing \eqref{eq:our-CE} instead allows to regularizing the predictions of the network for the background, thus avoiding to (i) experience a severe forgetting and (ii) to have a fixed and sub-optimal background representation.

\myparagraph{Revisiting Distillation Loss.}
To account for the background in a principled way, we also propose to revise the distillation loss. % to this scenario means to explicitly taking into account the fact that our semantic knowledge is shifting after each learning step.
In the considered setting, we should take into account the fact that at each learning step what was previously labeled as background may belong to the semantic class we are currently aiming to learn. As a consequence, the probability of the background class estimated through the old predictor $f_{\theta^{t-1}}$ does not correspond to the probability obtained with $f_{\theta^{t}}$, due to the inherent semantic shift of the background class. Notice that this aspect is peculiar to the segmentation task and it is not considered in previous incremental learning models for image-level classification. However, in our setting it must explicitly take it into account in order to perform a correct distillation of the old model into the new one. To this extent we define our novel distillation loss as: % During an incremental learning learning the new classifier we must take into account the semantic shift of 
%Since the class background changes form incremental step to incremental step, we cannot perform simple pixel-wise distillation on it. We can thus either ignore it, which is a suboptimal solution, or comparing the probability of the old background with the probability of the new background and the new classes. We modify distillation in such way:
\begin{equation}
    \label{eq:our-distill}
    \ell_{ukd}(x)=\sum_{k \in \mathcal{{Y}}^{t-1}} q_{t-1}(x)_k \log \hat{q}_t(x)_k 
\end{equation}
where:
\begin{equation}
    \label{eq:cases-distill}
    \begin{cases}
      \hat{q}_t(x)_k={q}_t(x)_k\;\;& \text{if}\ k\neq\mathtt{b}\\
      \hat{q}_t(x)_k= \sum_{c\in\{\mathcal{C}^t,\mathtt{b}\}}{q}_t(x)_c\;\;& \text{if}\ k=\mathtt{b}
    \end{cases}
\end{equation}
Similarly to Eq.\eqref{eq:std-distill}, in Eq. \eqref{eq:our-distill} we compare the probability of previously learned classes, obtained with the old model, with its counterpart computed with the current parameters $\theta_t$. However, differently from classical distillation, in Eq.\eqref{eq:our-distill}, the logits obtained with the current model are normalized across the whole output space \ie $\mathcal{{Y}}^t$ and not with respect to $\mathcal{{Y}}^{t-1}$. More importantly, the background class of $f_{\theta_{t-1}}$ is not directly compared with its counterpart in $f_{\theta_t}$, but with the probability of having \textit{either a new class or the background}, as predicted by $f_{\theta_t}$. This allows to propagate the uncertainty of the old parameters regarding the actual semantic content of the background by not penalizing the probabilities of the new classes we are trying to learn in the current incremental learning step $t$. %TODO\textcolor{red}{Finally, we would like to remark that Eq. \eqref{eq:our-distill} is the counterpart of Eq. \eqref{eq:our-CE}, when the ground truth label $y$ is replaced by the old model predictions $q_{t-1}$, producing an elegant solution to the semantic shift of $\mathtt{b}$ and the catastrophic forgetting problem.}

%$\hat{q}_n^t(x)_k={q}_n^t(x)_k$ if $k \neq b$ but, in case of the background, it is defined as:
% \begin{equation}
%       \hat{p}_b^n(x)  = \sum_{c\in \{\mathcal{N},b\}}p_c^n(x)
% \end{equation}


\myparagraph{Classifiers' Parameters Initialization.} As discussed above, when the current classification models is not able to assign a pixel to any known object class, it outputs the background label $\mathtt{b}$. In practice, at each learning step $t$, the novel categories in $\mathcal{C}^t$ are unknowns for the old classifier $f_{\theta^{t-1}}$. As a consequence, unless the appearance of a class in $\mathcal{C}^t$ is very similar to one in $\mathcal{Y}^{t-1}$, it is reasonable to assume that $f_{\theta^{t-1}}$ will likely assign the novel categories to the background. Taking into account this initial training bias for $\mathcal{C}^t$, it is detrimental to randomly initialize the classifiers for the novel classes, since we would risk a misalignment among the features extracted by the model (biased towards $\mathtt{b}$) and the parameters (random) of the classifier itself. Notice also that this could lead to possible training instabilities which we would like to avoid.% could lead to possible training instabilities. In fact, since the features extracte by the old model for the ntends to extract features  since the initial predictions for novel classes would be inherently unaligned with the features extracted by the old model, leading to possible training instabilities. %While this might not always happen (\eg the appearance of some images corresponding to class in $\mathcal{C}^t$ is very similar to those of one of the classes in $\mathcal{Y}^{t-1}$), \textcolor{red}{in our scenario is more probable since we assume the possibility of having pixels of classes in $\mathcal{C}^t$ labeled as background in the previous learning step. Taking into account this initial training bias for novel classes, it is detrimental to randomly initialize the classifiers for the novel classes since it would (i) not respect the priors given by the actual problem statement and (ii) lead to possible training instabilities}.  

To address this issue, we propose to explicitly align the classifiers for the novel classes in $\mathcal{C}^t$ to the old background classifier. To this extent, we initialize the classifiers of the novel classes in such a way that given an image $x$, the probability of the background for $f_{\theta_{t-1}}(x)$ is uniformly spread, initially, among $\mathcal{C}^{t}$ and $\mathtt{b}$ in $f_{\theta_t}(x)$. Let us write the classifier parameters for a class $c$ and a learning step $t$ as $\{\omega_{t}^c, \beta^{t}_c\}$ with $\omega^c$ and $\beta_c$ denoting the weights and the bias respectively. We can initialize $\{\omega^t_c, \beta^t_c\}$ as follows:
%Let us denote as $\mathcal{M}$ the set of old classes, $\mathcal{N}$ the set of new classes and $b$ as the background. Let as also define the probability of the input features x to belong to the class c as:
%\begin{equation}
%    p_\Theta(c|x)= p_c(x)=e^{\theta_c^\intercal x + \beta_c}
%\end{equation}
% where $\theta_c$ are the weights of the classifier for class $c$ and $\beta_c$ the relative bias. Let us also denote as $\Theta^n$ the parameters of the new classifier and $\Theta^o$ the parameters of the old model. In the following $p_c^o(x)$ would denote the probability of having class $c$ for the old model given $x$ and similarly $p_c^n(x)$ will denote the same probability but given by the new model.
% We base our method on 2 assumptions: 
% \begin{itemize}
%     \item Since in the first incremental step, $b$ could have contained also future classes we assume that:\\ $ p^o_b(x)= p^n_b(x)+\sum_{c\in N}p^n_c(x)$
%     \item Similarly, since the new set of images might contain old classes as unknown, we assume that:\\ $p^n_b(x)= p^n_b(x)+\sum_{c\in M}p^n_c(x)$
% \end{itemize}
% Given these two formulations we derive an approach based on:
% \begin{itemize}
%     \item Uniform initialization for the new classes given the background
%     \item A distillation term which is rebalanced by merging the probabilities of new classes and background
%     \item A cross-entropy term which is rebalanced by merging the probabilities of old classes and background
% \end{itemize}
% Since new classes are unknown to the old classifier ($\Theta_{o}$), we take this into account by initializing the classifiers of the new classes in such a way that they are aligned with the old background classifier. In particular we initialize the new classifier $\Theta_{n}$ in this way:
\begin{equation}
    \label{eq:init-cases}
    \begin{cases}
      \omega_c^{t}=\omega^{t-1}_c \;\;\text{and}\;\; \beta_c^{t}=\beta_c^{t},\;\;\;\;\;\;\;\;\;\;\;\; \text{if}\ c \in \mathcal{Y}^{t-1}\wedge c\neq\mathtt{b}\\
      \omega_c^{t}=\omega_\mathtt{b}^{t-1} \;\;\text{and}\;\; \beta_{t}^c=\beta_\mathtt{b}^{t-1} - \log(|\mathcal{C}^t|),\;\;\;\;\;\;\;\; \text{if}\ c \in \mathcal{C}^t\\
    \end{cases}
\end{equation}
where $|\mathcal{C}^t|$ is the number of new classes (notice that $\mathtt{b} \in \mathcal{C}^t$) and $\{\omega_\mathtt{b}^{t-1},\beta_\mathtt{b}^{t-1} \}$ are the weights and bias of the background classifier at the previous learning step. The second case of \eqref{eq:init-cases} can be simply derived by just uniformly dividing the probability of $\mathtt{b}$ from the old classifier among the new classes and $\mathtt{b}$, \ie: 
\begin{equation}
      \label{eq:init-derivation}
      q_{t-1}(x)_\mathtt{c} \propto \frac{e^{\omega_\mathtt{b}^{t-1}\cdot x + \beta^{t-1}_\mathtt{b}}}{|\mathcal{C}^t|}=e^{\omega_\mathtt{b}^{t-1}\cdot x + \beta^{t-1}_\mathtt{b}-\log(|\mathcal{C}^t|)}
\end{equation}
for $c \in \mathcal{{C}}^t$.

As we will show in the experimental analysis (\massi{TODO}) this simple initialization procedure does not only bring benefits in terms of training stability but also in terms of performances, since it follows the same principles used to define our distillation loss (Eq. \eqref{eq:our-distill}).


% \textbf{Implementation details}: For practical reasons, we can rewrite the loss relative to the background with two \textit{logsumofexps}:
% \begin{align}
%     L_{ukd}(x,b)&= p_b^o(x) \log \sum_{i\in \{\mathcal{N},b\}}e^{\theta_i^{n\;\intercal} x + \beta^n_i}\\ &- p_b^o(x) \log \sum_{j\in \{\mathcal{M},\mathcal{N},b\}}e^{\theta_j^{n\;\intercal} x + \beta^n_j}
% \end{align}



==> trash.tex <==
\fabio{Da RIMUOVERE Fino a ... }

\textbf{Ours-EXC} is an additional model that refers to a special case in which we perform classification only on pixels of new classes and distillation only on background pixels. Putting it into formulas:
\begin{equation}
    L_{exc}(x) = (1-y_{b}) \cdot L_{ce}(x) +  \lambda y_{b} \cdot L_{ukd}(x)  
\end{equation}

\textit{only BG} refers to the case where we do not consider pixels belonging to new classes in the distillation, i.e. by computing the loss only on the pixels whose ground truth is background. It's important to underline that instead of averaging over all pixels, the cumulative loss is obtained as:
\begin{equation}
    L_d^{bkg} = \frac{1}{|P_o|} \sum_{x \in P_o} L_d(x),
\end{equation}
where $P_o = \{x: x \in P, gt(p)=bkg \}$ is the set of pixels whose ground truth is background, and $P$ is the set of all pixels. Notice that here $L_d$ is a generic distillation loss, which can be also our $L_{ukd}$.

Moreover, we report an additional baseline that is \textit{Pseudo} which refers to a model that substitute the background label in the ground truth with the prediction of the old model and then perform the Cross Entropy Loss on this new ground truth. The pixel-wise loss thus become:
\begin{equation}
    L_{ps}(x) = y_{b}\cdot\sum_{j \in \{\mathcal{M}, b \}} q^{max}_j \log p_j(x) + \sum_{k \in \{ \mathcal{N},\mathcal{M} \} } y_k \log p_k(x),
\end{equation}
where $q^{max}$ represent the one-hot vector built on the argmax of the prediction of the old model, $y_k$ the one-hot of the ground-truth.

\fabio{Qui}

%\ding{51}
\begin{table*}[b]
\caption{\textbf{Main Ablation VOC}}
\begin{tabular}{l|cccc|cc|cc|cc|cc}
&\multicolumn{4}{c|}{ Choices}&\multicolumn{2}{c|}{15-5 ov.}&\multicolumn{2}{c|}{15-5 m.} & \multicolumn{2}{c}{15-5 s. ov. m.} & \multicolumn{2}{c}{15-5 s. m.}\\
\textbf{Method} &init &only BG & KD& CE     &  mAcc     & mIoU      & mAcc      & mIoU      & mAcc      & mIoU      & mAcc      & mIoU          \\ \hline
Offline &\multicolumn{4}{c|}{ }             &  86.1     & 78.2      & 86.1      & 78.2      &  86.1     & 78.2      & 86.1      & 78.2          \\ \hline
Ours-UKD  & & & \tick &                     &           &	        &           & 	        & 	        &           &           &               \\ 
Ours-UKD  &  & \tick & \tick &              & 77.0      & 62.3      & 80.3      & 66.2      &           &           &           &               \\
Ours-UKD  & \tick & \tick & \tick&          & 79.2      & 65.7      & 77.7      & 63.4      &           &           &           &               \\
Ours-UKD  & \tick & & \tick &               & 80.4      & 68.3      & 76.8      & 62.9      & 15.0      &  9.5      &  19.2     & 13.2          \\
Ours-EXC  & \tick & \tick & &               & 76.4      & 50.1      & 71.6      & 44.9	    & 	        &           &           &               \\
Ours-UCE  & \tick & & &\tick                & 75.8      & 59.2      &           & 	        & 	        &           &           &               \\
LwF-UCE   & & & & \tick                     & 76.0      & 59.8	    & 76.8      & 60.8	    & 18.0      &  10.5     &  16.7     & 9.2           \\
Ours-SYM  & & &\tick &\tick                 &	        &           & 	        &           & 	        &           &           &               \\ 
Ours-SYM  & & \tick &\tick &\tick           & 81.5      & 65.4      & \bf{82.9}	& \bf{67.2}	& 	        &           &           &               \\ 
Ours-SYM  & \tick & \tick &\tick &\tick     & 83.9      & 69.1      & 81.2      & 64.8      &           &           &           &               \\
Ours-SYM  & \tick &  & \tick & \tick        & \bf{84.5} & \bf{70.0} & {81.9}    & {65.3}    & 45.1      &  32.1     &  52.9     &  39.9         \\       
\end{tabular}
\end{table*}

\begin{table*}[b]
\caption{\textbf{Main Ablation ADE}}
\begin{tabular}{l|cccc|cc|cc|cc}
&\multicolumn{4}{c|}{ Choices}&\multicolumn{2}{c|}{100-50}&\multicolumn{2}{c|}{100-10 seq} & \multicolumn{2}{c}{50 seq}\\
\textbf{Method} &init &only BG & KD& CE     &  mAcc     & mIoU      & mAcc      & mIoU      & mAcc      & mIoU          \\ \hline
Offline &\multicolumn{4}{c|}{ }              & 47.5     & 38.9      &           &           &           &               \\ \hline
Ours-UKD  & & & \tick &                      & 23.1	    & 21.3	    &           &           &           &               \\ 
Ours-UKD  &  & \tick & \tick &               &          &           &           &           &           &               \\
Ours-UKD  & \tick & \tick & \tick&           & 23.4     & 21.0      &           &           &           &               \\
Ours-UKD  & \tick & & \tick &                & 22.0     & 20.4      &           &           &           &               \\
Ours-EXC  & \tick & \tick & &                & 49.6	    & 32.1	    &           &           &           &               \\
Ours-UCE  & \tick & & &\tick                 & 36.1	    & 28.3	    &  31.1     &  19.8     &           &               \\
LwF-UCE   & & & & \tick                      & 44.1	    & 34.6      &  32.7     &  26.2     & 37.4      &  28.8         \\
Ours-SYM  & & &\tick &\tick                  & 43.9	    & 34.9	    &  34.8     &  27.2     &           &               \\                                                   
Ours-SYM  & & \tick &\tick &\tick            & 44.0	    & 34.8      &  33.7     &  26.5     &           &               \\ 
Ours-SYM  & \tick & \tick &\tick &\tick      &          &	        & \bf{38.3} & \bf{28.4} &           &               \\
Ours-SYM  & \tick &  & \tick & \tick         & \bf{46.1}& \bf{35.0} &  37.5     & 27.6      & 37.6      &  27.9         \\       
\end{tabular}
\end{table*}

\begin{table*}[b]
\caption{VOC 19-1 masked TODO}
\begin{tabular}{l|cccc|cccc}
Method                  & MA    & MA new    & MA old    & Harm. MA  & MIoU      & MIoU new  & MIoU old  & Harm. MIoU    \\ \hline
Joint (20)              & 86.1  &           &           &           &   78.2    &           &           &               \\ \hline
FT-CE (19)              &       &           &           &           &           &           &           &               \\ \hline
FT                      & 13.8  &	79.6    &	10.5    &	18.5    &	9.2     &	12.3    &	9.1     &	10.4        \\
Pseudo                  &       &           &           &           &           &           &           &               \\
KD                      & 59.3  &	79.9    &	58.2    &	67.4    &	52.6    &	9.1     &   54.7    &	15.7        \\ 
DE .                    & 23.8  &	72.8    &	21.4    &	33.1    &	20.1    &	21.7    &	20.0    &	20.8        \\ 
EWC                     & 29.6  &	75.3    &	27.3    &	40.1    &	25.3    &	16.0    &	25.8    &	19.7        \\ 
RW                      & 26.1  &	76.4    &	23.6    &	36.1    &	21.8    &	15.7    &	22.1    &	18.4        \\ 
PI                      & 13.5  &	82.1    &	10.1    &	18.0    &	8.9     &   14.1    & 	8.7     &	10.8        \\ 
ICaRL                   & 55.8  &	74.0    &	54.9    &	63.0    &	50.6    &	16.9    &	52.3    &	25.5        \\ \hline
\textbf{SYM}            &       &           &           &           &           &           &           &               \\ \hline
KD 5 exemplars          & 78.4  &	80.5    &	78.3    &	79.4    &	69.8    &	21.9    &	72.2    &	33.6        \\ 
EWC 5 exemplars         & 61.9  &	76.0    &	61.2    &	67.8    &	55.8    &	20.0    &	57.6    &	29.6        \\ 
ICaRL 5 exemplars       & 74.8  &	74.5    &	74.8    &	74.7    &	67.4    &	33.2    &	69.1    &	44.9        \\ \hline
KD 20 exemplars         & 83.9  &	79.6    &	84.1    &	81.8    &	74.4    &	36.4    &	76.3    &	49.2        \\
EWC 20 exemplars        & 75.7  &	73.6    &	75.8    &	74.7    &	67.7    &	32.4    &	69.4    &	44.2        \\
ICaRL 20 exemplars      & 81.3  &	72.9    &	81.7    &	77.0    &	73.0    &	46.7    &	74.3    &	57.3        
\end{tabular}
\end{table*}

\begin{table*}[b]
\caption{VOC 15-5 masked}
\begin{tabular}{l|cccc|cccc}
Method                  & MA    & MA new    & MA old    & Harm. MA  & MIoU      & MIoU new  & MIoU old  & Harm. MIoU    \\ \hline
Joint (20)              & 86.1  &           &           &           &   78.2    &           &           &               \\ \hline
FT (15)                 & 89.3  &           &           &           &   80.4    &           &           &               \\ \hline
FT                      & 25.9  &	86.2    &	 7.0    &	13.0    &	12.3    &	33.6    &	 5.7    &	 9.8        \\
Pseudo                  & 73.9  &	86.3    &	70.0    &	77.3    &	55.8    &	37.2    &	61.6    &	46.4        \\
KD                      & 70.6  &	87.2    &	65.5    &	74.8    &	54.9    &	37.4    &	60.4    &	46.2        \\ 
DE                      & 26.5  &	81.9    &	 9.1    &	16.4    &	14.7    &	37.0    &	 7.7    &	12.8        \\ 
EWC                     & 43.3  &	80.6    &	31.7    &	45.5    &	31.8    &	37.7    &	29.9    &	33.3        \\ 
RW                      & 37.2  &	82.1    &	23.2    &	36.2    &	25.3    &	36.9    &	21.6    &	27.3        \\ 
PI                      & 26.1  &	86.3    &	 7.2    &	13.4    &	12.6    &	34.1    &	 5.9    &	10.1        \\ 
ICaRL                   & 66.4  &	78.9    &	62.5    &	69.7    &	55.7    &	45.8    &	58.7    &	51.5        \\ \hline
\textbf{SYM}            & 81.9  &	81.3    & 	82.2    &	81.7    &	65.9    &	43.3    &	73.0    &	54.4        \\ \hline
KD 5 exemplars          & 76.3  &	87.3    &	72.8    &	79.4    &	61.2    &	42.7    &	67.0    &	52.1        \\ 
EWC 5 exemplars         & 50.9  &	80.1    &	41.8    &	55.0    &	39.7    &	39.8    &	39.7    &	39.7        \\ 
ICaRL 5 exemplars       & 73.4  &	79.5    &	71.5    &	75.3    &	63.1    &	51.2    &	66.9    &	58.0        \\ \hline
KD 20 exemplars         & 82.7  &	85.8    &	81.7    &	83.7    &	69.3    &	51.5    &	74.9    &	61.0        \\
EWC 20 exemplars        & 64.3  &	79.2    &	59.6    &	68.0    &	54.2    &	47.9    &	56.1    &	51.7        \\
ICaRL 20 exemplars      & 79.5  &	76.1    &	80.6    &	78.3    &	71.1    &	59.9    &	74.6    &	66.4        
\end{tabular}
\end{table*}

\begin{table*}[b]
\caption{VOC 15-5 overlapped/masked}
\begin{tabular}{l|cccc|cccc}
\textbf{Method}         & MA    & MA new   & MA old    & Harm. MA  & MIoU      & MIoU new  & MIoU old  & Harm. MIoU    \\ \hline
Joint (20)              & 86.1  &           &           &           &   78.2    &           &           &               \\ \hline
FT (15)                 & 87.9  &           &           &           &   79.9    &           &           &               \\ \hline
FT                      & 26.7  &	87.0    &	 7.9    &	14.5    &	12.9    &	33.1    &	 6.6    &	11.0        \\
Pseudo                  & 72.0  &	87.5    &	67.2    &	76.0    &	54.7    &	35.0    &	60.8    &	44.4        \\
KD                      & 70.3  &	87.2    &	64.9    &	74.5    &	55.0    &	36.6    &	60.8    &	45.7        \\ 
DE                      & 29.9  &	82.2    &	13.6    &	23.3    &	18.9    &	40.6    &	12.1    &	18.7        \\ 
EWC                     & 41.9  &	81.5    &	29.5    &	43.3    &	29.5    &	35.5    &	27.6    &	31.0        \\ 
RW                      & 36.5  &	83.2    &	22.0    &	34.7    &	23.8    &	34.9    &	20.3    &	25.7        \\ 
PI                      & 26.3  &	86.7    &	 7.5    &	13.8    &	12.6    &	33.3    &	 6.1    &	10.4        \\ 
ICaRL                   & 64.5  &	39.5    &	72.3    &	51.1    &	57.3    &	26.1    &	67.0    &	37.5        \\ \hline
\textbf{SYM}            & 84.5  &	85.1    &	84.3    &	84.7    &	70.0    &	49.4    &	76.4    &	60.0        \\\hline
KD 5 exemplars          & 76.9  &	87.4    &	73.7    &	79.9    &	62.8    &	43.2    &	68.9    &	53.1        \\ 
EWC 5 exemplars         & 50.6  &	81.3    &	41.0    &	54.5    &	38.7    &	39.8    &	38.3    &	39.0        \\ 
ICaRL 5 exemplars       & 69.9  &	40.9    &	79.0    &	53.9    &	63.1    &	30.6    &	73.3    &	43.2        \\ \hline
KD 20 exemplars         & 82.6  &	87.0    &	81.2    &	84.0    &	69.6    &	52.2    &	75.0    &	61.5        \\
EWC 20 exemplars        & 63.0  &	80.1    &	57.6    &	67.0    &	52.0    &	47.4    &	53.4    &	50.2        \\
ICaRL 20 exemplars      & 71.0  &	36.6    &	81.8    &	50.6    &	64.9    &	32.3    &	75.2    &	45.2          
\end{tabular}
\end{table*}

\begin{table*}[b]
\caption{ADE 100-50}
\begin{tabular}{l|cccc|cccc}
Method                  & MA        & MA new    & MA old    & Harm. MA  &   MIoU    & MIoU new  & MIoU old  & Harm. MIoU        \\ \hline
Joint (150)             &   47.5      &	33.9    &  54.3     &		    &   38.9    &	28.2    &	44.3    &	                \\ \hline
FT (100)                &   52.7      &           &           &           &   42.6    &           &           &                 \\ \hline
FT                      &    8.0    &	23.9    &	 0.0    &	 0.0    &	 6.2    &	18.7    &	 0.0    &	 0.0            \\ 
FT unmasked             &   40.7    &	27.3    &	47.5    &	34.6    &	32.5    &	19.4    &	39.0    &	25.9            \\ 
PSEUDO                  &   42.9    &	25.6    &	51.5    &	34.2    &	34.2    &	19.2    &	41.7    &	26.3            \\ 
KD                      &   24.5    &	23.6    &	25.0    &	24.3    &	21.8    &	18.2    &	23.6    &	20.5            \\ 
EWC                     &   1.6     &	4.6     &	0.1     &	0.1     &	1.2     &	3.5     &	0.1     &	0.1             \\ 
RW                      &   2.6     &	7.2     &	0.3     &	0.5     &	2.1     &	5.7     &	0.3     &	0.5             \\ 
PI                      &    8.1    &	24.3    &	 0.0    &	 0.0    &	 6.5    &	19.5    &	 0.0    &	 0.0            \\ 
ICaRL                   &   20.2    &	16.0    &	22.3    &	18.6    &	18.2    &	11.9    &	21.3    &	15.3            \\ \hline
\textbf{SYM}            &   46.1    &	30.8    &	53.8    &	39.1    &	35.0    &	22.1    &	41.5    &	28.8            \\ \hline
KD 5 exemplars          &        &        &	      &          &      &	       &          &             \\ 
EWC 5 exemplars         &        &        &	      &          &      &	       &          &             \\ 
ICaRL 5 exemplars       &        &        &	      &          &      &	       &          &             \\ \hline
KD 20 exemplars         &        &        &	      &          &      &	       &          &             \\
EWC 20 exemplars        &        &        &	      &          &      &	       &          &             \\
ICaRL 20 exemplars      &        &        &	      &          &      &	       &          &             
\end{tabular}
\end{table*}
